Metastability for the degenerate Potts Model with positive external magnetic field under Glauber dynamics

We consider the ferromagnetic q-state Potts model on a finite grid graph with non-zero external field and periodic boundary conditions. The system evolves according to Glauber-type dynamics described by the Metropolis algorithm, and we focus on the low temperature asymptotic regime. We analyze the case of positive external magnetic field. In this energy landscape there are $1$ stable configuration and $q-1$ metastable states. We study the asymptotic behavior of the first hitting time from any metastable state to the stable configuration as $\beta\to\infty$ in probability, in expectation, and in distribution. We also identify the exponent of the mixing time and find an upper and a lower bound for the spectral gap. We also geometrically identify the union of all minimal gates and the tube of typical trajectories for the transition from any metastable state to the unique stable configuration.

==> mybib.tex <==
@article{manzo2004essential,
  title={On the essential features of metastability: tunnelling time and critical configurations},
  author={Manzo, Francesco and Nardi, Francesca R and Olivieri, Enzo and Scoppola, Elisabetta},
  journal={Journal of Statistical Physics},
  volume={115},
  number={1-2},
  pages={591--642},
  year={2004},
  publisher={Springer}
}
@article{alonso1996three,
  title={The three dimensional polyominoes of minimal area},
  author={Alonso, Laurent and Cerf, Rapha{\"e}l},
  journal={The Electronic Journal of Combinatorics},
  volume={3},
  number={1},
  pages={R27},
  year={1996}
}
@book{olivieri2005large,
  title={Large deviations and metastability},
  author={Olivieri, Enzo and Vares, Maria Eul{\'a}lia},
  volume={100},
  year={2005},
  publisher={Cambridge University Press}
}
@article{nardi2019tunneling,
  title={Tunneling behavior of {I}sing and {P}otts models in the low-temperature regime},
  author={Nardi, Francesca R and Zocca, Alessandro},
  journal={Stochastic Processes and their Applications},
  volume={129},
number={11},
  pages={4556--4575},
  year={2019},
  publisher={Elsevier}
}
@article{nardi2016hitting,
  title={Hitting time asymptotics for hard-core interactions on grids},
  author={Nardi, Francesca R and Zocca, Alessandro and Borst, Sem C},
  journal={Journal of Statistical Physics},
  volume={162},
  number={2},
  pages={522--576},
  year={2016},
  publisher={Springer}
}
@article{kac1963van,
  title={On the van der Waals Theory of the Vapor-Liquid Equilibrium. I. Discussion of a One-Dimensional Model},
  author={Kac, M and Uhlenbeck, GE and Hemmer, PC},
  journal={Journal of Mathematical Physics},
  volume={4},
  number={2},
  pages={216--228},
  year={1963},
  publisher={American Institute of Physics}
}
@article{cassandro1984metastable,
  title={Metastable behavior of stochastic dynamics: a pathwise approach},
  author={Cassandro, Marzio and Galves, Antonio and Olivieri, Enzo and Vares, Maria Eul{\'a}lia},
  journal={Journal of Statistical Physics},
  volume={35},
  number={5},
  pages={603--634},
  year={1984},
  publisher={Springer}
}
@article{cirillo2013relaxation,
  title={Relaxation height in energy landscapes: an application to multiple metastable states},
  author={Cirillo, Emilio NM and Nardi, Francesca R},
  journal={Journal of Statistical Physics},
  volume={150},
  number={6},
  pages={1080--1114},
  year={2013},
  publisher={Springer}
}
@inproceedings{potts1952some,
  title={Some generalized order-disorder transformations},
  author={Potts, Renfrey Burnard},
  booktitle={Mathematical proceedings of the cambridge philosophical society},
  volume={48},
  number={1},
  pages={106--109},
  year={1952},
  organization={Cambridge University Press}
}
@article{olivieri1995markov,
  title={Markov chains with exponentially small transition probabilities: first exit problem from a general domain. The reversible case},
  author={Olivieri, Enzo and Scoppola, Elisabetta},
  journal={Journal of Statistical Physics},
  volume={79},
  number={3},
  pages={613--647},
  year={1995},
  publisher={Springer}
}
@article{olivieri1996markov,
  title={Markov chains with exponentially small transition probabilities: first exit problem from a general domain. The general case},
  author={Olivieri, Enzo and Scoppola, Elisabetta},
  journal={Journal of Statistical Physics},
  volume={84},
  number={5},
  pages={987--1041},
  year={1996},
  publisher={Springer}
}
@article{penrose1971rigorous,
  title={Rigorous treatment of metastable states in the van der Waals-Maxwell theory},
  author={Penrose, Oliver and Lebowitz, Joel L},
  journal={Journal of Statistical Physics},
  volume={3},
  number={2},
  pages={211--236},
  year={1971},
  publisher={Springer}
}
@article{arous1996metastability,
  title={Metastability of the three dimensional {I}sing model on a torus at very low temperatures},
  author={Arous, G{\'e}rard Ben and Cerf, Rapha{\"e}l },
  journal={Electronic Journal of Probability},
  volume={1},
  year={1996},
  publisher={The Institute of Mathematical Statistics and the Bernoulli Society}
}
@article{cirillo1998metastability,
  title={Metastability in the two-dimensional {I}sing model with free boundary conditions},
  author={Cirillo, Emilio NM and Lebowitz, Joel L},
  journal={Journal of Statistical Physics},
  volume={90},
  number={1},
  pages={211--226},
  year={1998},
  publisher={Springer}
}
@article{cirillo1996metastability,
  title={Metastability and nucleation for the {B}lume-{C}apel model. {D}ifferent mechanisms of transition},
  author={Cirillo, Emilio NM and Olivieri, Enzo},
  journal={Journal of Statistical Physics},
  volume={83},
  number={3},
  pages={473--554},
  year={1996},
  publisher={Springer}
}
@article{hollander2000metastability,
  title={Metastability and nucleation for conservative dynamics},
  author={Hollander, F den and Olivieri, Enzo and Scoppola, Elisabetta},
  journal={Journal of Mathematical Physics},
  volume={41},
  number={3},
  pages={1424--1498},
  year={2000},
  publisher={American Institute of Physics}
}
@article{den2003droplet,
  title={Droplet growth for three-dimensional {K}awasaki dynamics},
  author={den Hollander, F and Nardi, FR and Olivieri, E and Scoppola, E},
  journal={Probability Theory and Related Fields},
  volume={125},
  number={2},
  pages={153--194},
  year={2003},
  publisher={Springer}
}
@article{gaudilliere2005nucleation,
  title={Nucleation pattern at low temperature for local {K}awasaki dynamics in two dimensions},
  author={Gaudilliere, Alexandre and Olivieri, Enzo and Scoppola, Elisabetta},
  journal={Markov Processes and Related Fields},
  volume={11},
  pages={553--628},
  year={2005}
}
@article{kotecky1994shapes,
  title={Shapes of growing droplets—a model of escape from a metastable phase},
  author={Koteck{\`y}, R and Olivieri, E},
  journal={Journal of Statistical Physics},
  volume={75},
  number={3},
  pages={409--506},
  year={1994},
  publisher={Springer}
}
@inproceedings{nardi1996low,
  title={Low temperature stochastic dynamics for an {I}sing model with alternating field},
  author={Nardi, Francesca R and Olivieri, Enzo},
  booktitle={Markov Proc. Relat. Fields},
  volume={2},
  pages={117--166},
  year={1996}
}
@article{neves1991critical,
  title={Critical droplets and metastability for a {G}lauber dynamics at very low temperatures},
  author={Neves, E Jordao and Schonmann, Roberto H},
  journal={Communications in Mathematical Physics},
  volume={137},
  number={2},
  pages={209--230},
  year={1991},
  publisher={Springer}
}
@article{neves1992behavior,
  title={Behavior of droplets for a class of {G}lauber dynamics at very low temperature},
  author={Neves, E Jord{\~a}o and Schonmann, Roberto H},
  journal={Probability Theory and Related Fields},
  volume={91},
  number={3-4},
  pages={331--354},
  year={1992},
  publisher={Springer}
}
@article{cirillo2003metastability,
  title={Metastability for a stochastic dynamics with a parallel heat bath updating rule},
  author={Cirillo, Emilio NM and Nardi, Francesca R},
  journal={Journal of Statistical Physics},
  volume={110},
  number={1},
  pages={183--217},
  year={2003},
  publisher={Springer}
}
@article{cirillo2008competitive,
  title={Competitive nucleation in reversible probabilistic cellular automata},
  author={Cirillo, Emilio NM and Nardi, Francesca R and Spitoni, Cristian},
  journal={Physical Review E},
  volume={78},
  number={4},
  pages={040601},
  year={2008},
  publisher={APS}
}
@article{cirillo2008metastability,
  title={Metastability for reversible probabilistic cellular automata with self-interaction},
  author={Cirillo, Emilio NM and Nardi, Francesca R and Spitoni, Cristian},
  journal={Journal of Statistical Physics},
  volume={132},
  number={3},
  pages={431--471},
  year={2008},
  publisher={Springer}
}
@article{cirillo2015metastability,
  title={Metastability for general dynamics with rare transitions: escape time and critical configurations},
  author={Cirillo, Emilio NM and Nardi, Francesca R and Sohier, Julien},
  journal={Journal of Statistical Physics},
  volume={161},
  number={2},
  pages={365--403},
  year={2015},
  publisher={Springer}
}
@article{bovier2004metastability,
title={Metastability in reversible diffusion processes {I}. {Sharp} asymptotics for capacities and exit
times},
author={Bovier, Anton and Eckhoff, Michael and Gayrard, V{\'e}ronique and Klein, Markus},
journal={Journal of the European Mathematical Society},
year={2004}
}
@article{bianchi2016metastable,
title={Metastable states, quasi-stationary distributions and soft measures},
author={Bianchi, Alessandra and Gaudilliere, Alexandre},
journal={Stochastic Processes and their Applications},
volume={126},
number={6},
pages={1622--1680},
year={2016},
publisher={Elsevier}
}
@article{procacci2016probabilistic,
  title={Probabilistic Cellular Automata for Low-Temperature 2-d {I}sing Model},
  author={Procacci, Aldo and Scoppola, Benedetto and Scoppola, Elisabetta},
  journal={Journal of Statistical Physics},
  volume={165},
  number={6},
  pages={991--1005},
  year={2016},
  publisher={Springer}
}
@article{bet2020effect,
  title={Effect of energy degeneracy on the transition time for a series of metastable states: application to Probabilistic Cellular Automata},
  author={Bet, Gianmarco and Jacquier, Vanessa and Nardi, Francesca R},
  journal={arXiv:2007.08342},
  year={2020}
}
@article{bashiri2017note,
  title={A note on the metastability in three modifications of the standard {{I}sing} model},
  author={Bashiri, Kaveh},
  journal={arXiv:1705.07012},
  year={2017}
}
@article{bashiri2019on,
title={On the Metastability in Three Modifications of the {I}sing model},
  author={Bashiri, Kaveh},
  journal={View Journal Impact},
  volume={25},
  number={3},
  pages={483--532},
  year={2019}
}
@article{beltran2010tunneling,
  title={Tunneling and metastability of continuous time {M}arkov chains},
  author={Beltran, Johel and Landim, Claudio},
  journal={Journal of Statistical Physics},
  volume={140},
  number={6},
  pages={1065--1114},
  year={2010},
  publisher={Springer}
}

@article{beltran2012tunneling,
  title={Tunneling and metastability of continuous time {M}arkov chains, the nonreversible case},
  author={Beltr{\'a}n, J and Landim, C},
  journal={Journal of Statistical Physics},
  volume={149},
  number={4},
  pages={598--618},
  year={2012},
  publisher={Springer}
}

@article{gaudillierelandim2014,
  TITLE = {{A Dirichlet principle for non reversible Markov chains and some recurrence theorems}},
  AUTHOR = {Gaudilliere, Alexandre and Landim, Claudio},
  JOURNAL = {{Probability Theory and Related Fields}},
  PUBLISHER = {{Springer Verlag}},
  VOLUME = {158},
  PAGES = {55-89},
  YEAR = {2014}
}


@article{fernandez2015asymptotically,
  title={Asymptotically exponential hitting times and metastability: a pathwise approach without reversibility},
  author={Fernandez, Roberto and Manzo, Francesco and Nardi, Francesca and Scoppola, Elisabetta},
  journal={Electronic Journal of Probability},
  volume={20},
  year={2015},
  publisher={The Institute of Mathematical Statistics and the Bernoulli Society}
}

@article{fernandez2016conditioned,
  title={Conditioned, quasi-stationary, restricted measures and escape from metastable states},
  author={Fernandez, Roberto and Manzo, Francesco and Nardi, FR and Scoppola, Elisabetta and Sohier, Julien },
  journal={Annals of Applied Probability},
  volume={26},
  number={2},
  pages={760--793},
  year={2016},
  publisher={Institute of Mathematical Statistics}
}
@article{jovanovski2017metastability,
  title={Metastability for the {I}sing Model on the hypercube},
  author={Jovanovski, Oliver},
  journal={Journal of Statistical Physics},
  volume={167},
  number={1},
  pages={135--159},
  year={2017},
  publisher={Springer}
}
@article{bovier2006sharp,
  title={Sharp asymptotics for {K}awasaki dynamics on a finite box with open boundary},
  author={Bovier, Anton and den Hollander, Frank and Nardi, Francesca R},
  journal={Probability Theory and Related Fields},
  volume={135},
  number={2},
  pages={265--310},
  year={2006},
  publisher={Springer}
}
@article{cirillo2017sum,
  title={Sum of exit times in a series of two metastable states},
  author={Cirillo, Emilio NM and Nardi, Francesca R and Spitoni, Cristian},
  journal={The European Physical Journal Special Topics},
  volume={226},
  number={10},
  pages={2421--2438},
  year={2017},
  publisher={Springer}
}
@article{nardi2012sharp,
  title={Sharp asymptotics for stochastic dynamics with parallel updating rule},
  author={Nardi, FR and Spitoni, C},
  journal={Journal of Statistical Physics},
  volume={146},
  number={4},
  pages={701--718},
  year={2012},
  publisher={Springer}
}
@book{bovier2016metastability,
  title={Metastability: a potential-theoretic approach},
  author={Bovier, Anton and Den Hollander, Frank},
  volume={351},
  year={2016},
  publisher={Springer}
}
@article{boviermanzo2002metastability,
  title={Metastability in {{G}lauber} dynamics in the low-temperature limit: beyond exponential asymptotics},
  author={Bovier, Anton and Manzo, Francesco},
  journal={Journal of Statistical Physics},
  volume={107},
  number={3-4},
  pages={757--779},
  year={2002},
  publisher={Springer}
}
@article{den2012metastability,
  title={Metastability for {K}awasaki dynamics at low temperature with two types of particles},
  author={den Hollander, Frank and Nardi, Francesca and Troiani, Alessio},
  journal={Electronic Journal of Probability},
  volume={17},
  year={2012},
  publisher={The Institute of Mathematical Statistics and the Bernoulli Society}
}
@article{apollonio2021metastability,
  title={Metastability for the {I}sing model on the hexagonal lattice},
  author={Apollonio, Valentina and Jacquier, Vanessa and Nardi, Francesca Romana and Troiani, Alessio},
  journal={arXiv:2101.11894},
  year={2021}
}
@article{bovier2002metastability,
  title={Metastability and Low Lying Spectral in Reversible {M}arkov Chains},
  author={Bovier, Anton and Eckhoff, Michael and Gayrard, V{\'e}ronique and Klein, Markus},
  journal={Communications in Mathematical Physics},
  volume={228},
  number={2},
  pages={219--255},
  year={2002},
  publisher={Springer}
}
@article{dai2015fast,
  title={Fast mixing for the low temperature 2D {I}sing model through irreversible parallel dynamics},
  author={Dai Pra, Paolo and Scoppola, Benedetto and Scoppola, Elisabetta},
  journal={Journal of Statistical Physics},
  volume={159},
  number={1},
  pages={1--20},
  year={2015},
  publisher={Springer}
}
@article{catoni1997exit,
  title={The exit path of a {M}arkov chain with rare transitions},
  author={Catoni, Olivier and Cerf, Rapha{\"e}l},
  journal={ESAIM: Probability and Statistics},
  volume={1},
  pages={95--144},
  year={1997}
}
@article{den2018metastability,
  title={Metastability of hard-core dynamics on bipartite graphs},
  author={den Hollander, Frank and Nardi, Francesca R and Taati, Siamak},
  journal={Electronic Journal of Probability},
  volume={23},
  year={2018},
  publisher={The Institute of Mathematical Statistics and the Bernoulli Society}
}
@article{zocca2019tunneling,
  title={Tunneling of the hard-core model on finite triangular lattices},
  author={Zocca, Alessandro},
  journal={Random Structures \& Algorithms},
  volume={55},
  number={1},
  pages={215--246},
  year={2019},
  publisher={Wiley Online Library}
}
@article{bet2021critical,
  title={Critical configurations and tube of typical trajectories for the {P}otts and {I}sing models with zero external field},
  author={Bet, Gianmarco and Gallo, Anna and Nardi, Francesca Romana},
  journal={Journal of Statistical Physics},
  volume={184},
  number={30},
  year={2021},
  publisher={Springer}
}
}
@article{baxter1973potts,
  title={Potts model at the critical temperature},
  author={Baxter, Rodney J},
  journal={Journal of Physics C: Solid State Physics},
  volume={6},
  number={23},
  pages={L445},
  year={1973},
  publisher={IOP Publishing}
}
@article{baxter1982critical,
  title={Critical antiferromagnetic square-lattice {P}otts model},
  author={Baxter, RJ},
  journal={Proceedings of the Royal Society of London. A. Mathematical and Physical Sciences},
  volume={383},
  number={1784},
  pages={43--54},
  year={1982},
  publisher={The Royal Society London}
}
@article{baxter1978triangular,
  title={Triangular {P}otts model at its transition temperature, and related models},
  author={Baxter, Rodney James and Temperley, HNV and Ashley, Susan E},
  journal={Proceedings of the Royal Society of London. A. Mathematical and Physical Sciences},
  volume={358},
  number={1695},
  pages={535--559},
  year={1978},
  publisher={The Royal Society London}
}
@article{enting1982triangular,
  title={Triangular lattice {P}otts models},
  author={Enting, IG and Wu, FY},
  journal={Journal of Statistical Physics},
  volume={28},
  number={2},
  pages={351--373},
  year={1982},
  publisher={Springer}
}
@article{ananikyan1995phase,
  title={Phase transition mechanisms in the {P}otts model on a {B}ethe lattice},
  author={Ananikyan, NS and Akheyan, AZ},
  journal={Journal of Experimental and Theoretical Physics},
  volume={80},
  number={1},
  pages={105--111},
  year={1995},
  publisher={New York, NY: American Institute of Physics, c1993-}
}
@article{de1991metastability,
  title={Metastability in the {P}otts model on the {C}ayley tree},
  author={de Aguiar, FS and Bernardes, LB and Rosa, S Goulart},
  journal={Journal of Statistical Physics},
  volume={64},
  number={3},
  pages={673--682},
  year={1991},
  publisher={Springer}
}
@article{di1987potts,
  title={The {P}otts model on {B}ethe lattices},
  author={di Liberto, F and Monroy, G and Peruggi, F},
  journal={Zeitschrift f{\"u}r Physik B Condensed Matter},
  volume={66},
  number={3},
  pages={379--385},
  year={1987},
  publisher={Springer}
}
@article{costeniuc2005complete,
  title={Complete analysis of phase transitions and ensemble equivalence for the {C}urie--{W}eiss--{P}otts model},
  author={Costeniuc, Marius and Ellis, Richard S and Touchette, Hugo},
  journal={Journal of Mathematical Physics},
  volume={46},
  number={6},
  pages={063301},
  year={2005},
  publisher={American Institute of Physics}
}
@article{ellis1990limit,
  title={Limit theorems for the empirical vector of the {C}urie-{W}eiss-{P}otts model},
  author={Ellis, Richard S and Wang, Kongming},
  journal={Stochastic Processes and their Applications},
  volume={35},
  number={1},
  pages={59--79},
  year={1990},
  publisher={Elsevier}
}
@article{ellis1992limit,
  title={Limit theorems for maximum likelihood estimators in the {C}urie-{W}eiss-{P}otts model},
  author={Ellis, Richard S and Wang, Kongming},
  journal={Stochastic Processes and their Applications},
  volume={40},
  number={2},
  pages={251--288},
  year={1992},
  publisher={Elsevier}
}
@article{gandolfo2010limit,
  title={Limit theorems and coexistence probabilities for the {C}urie-{W}eiss-{P}otts model with an external field},
  author={Gandolfo, Daniel and Ruiz, Jean and Wouts, Marc},
  journal={Stochastic Processes and their Applications},
  volume={120},
  number={1},
  pages={84--104},
  year={2010},
  publisher={Elsevier}
}
@article{wang1994solutions,
  title={Solutions of the variational problem in the {C}urie-{W}eiss-{P}otts model},
  author={Wang, Kongming},
  journal={Stochastic processes and their applications},
  volume={50},
  number={2},
  pages={245--252},
  year={1994},
  publisher={Elsevier}
}
@article{kim2021metastability,
  title={Metastability of Stochastic {I}sing and {P}otts Models on Lattices without External Fields},
  author={Kim, Seonwoo and Seo, Insuk},
  journal={arXiv:2102.05565},
  year={2021}
}
@inproceedings{bovier2006metastability,
  title={Metastability: a potential theoretic approach},
  author={Bovier, Anton and den Hollander, Frank},
  booktitle={International Congress of Mathematicians},
  volume={3},
  pages={499--518},
  year={2006},
  organization={Eur. Math. Soc. Z{\"u}rich}
}
@article{bet2021metastabilityneg,
  title={Metastability for the degenerate {P}otts {M}odel with negative external magnetic field under {G}lauber dynamics},
  author={Bet, Gianmarco and Gallo, Anna and Nardi, Francesca R},
  journal={arXiv:2105.14335}, 
  year={2021}
}
@article{baldassarri2021metastability,
  title={{C}ritical {D}roplets and sharp asymptotics for {K}awasaki dynamics with weakly anisotropic interactions},
  author={Baldassarri, Simone and Nardi, Francesca R},
  journal={arXiv:2108.02017},
  year={2021}
}
@article{bet2021metastabilitypos,
  title={Metastability for the degenerate {P}otts {M}odel with positive external magnetic field under {G}lauber dynamics},
  author={Bet, Gianmarco and Gallo, Anna and Nardi, Francesca R},
  journal={arXiv:2108.04011},
  year={2021}
}
